Robust Online Control with Model Misspecification

We study online control of an unknown nonlinear dynamical system that is approximated by a time-invariant linear system with model misspecification. Our study focuses on robustness, a measure of how much deviation from the assumed linear approximation can be tolerated by a controller while maintaining finite $\ell_2$-gain. A basic methodology to analyze robustness is via the small gain theorem. However, as an implication of recent lower bounds on adaptive control, this method can only yield robustness that is exponentially small in the dimension of the system and its parametric uncertainty. The work of Cusumano and Poolla shows that much better robustness can be obtained, but the control algorithm is inefficient, taking exponential time in the worst case. In this paper we investigate whether there exists an efficient algorithm with provable robustness beyond the small gain theorem. We demonstrate that for a fully actuated system, this is indeed attainable. We give an efficient controller that can tolerate robustness that is polynomial in the dimension and independent of the parametric uncertainty; furthermore, the controller obtains an $\ell_2$-gain whose dimension dependence is near optimal.

==> one_dimension.tex <==
\section{Tight bounds for One Dimensional Systems}\label{one_dim:sec}

We first consider a restricted setting, where the state is a scalar.  In particular, in this section we consider dynamics defined by equations
\begin{equation}\label{am1}  
x_{t+1}=ay_t+u_t+w_t+f_t,\quad 
|w_{0:t}|\le h|x_{0:t}|\quad\forall~t\in\mathbb Z_+,\quad x_0=0,
\end{equation}
where $a$ is the {\sl parametric uncertainty}, an unknown constant taking values from
a {\sl known} interval $a\in[-M,M]$.  

We prove two types of results: first, we show that, independently of
the adaptive controller used, the closed loop $\ltgain$ will
not be smaller than a certain lower bound, which grows linearly with the uncertainty radius $M$, even in the case when no non-parametric uncertainty is present ($h=0$). 
Second, we show that a well-known adaptive controller in fact does 
satisfy closed loop $\ltgain$ bounds which grow linearly with $M$, for every fixed $h<1/2$.

\subsection{Lower Bound}
First, we formulate (and prove) a stronger version of the result of \cite{megretzki_l2_gain},
for the case $h=0$ (which means that $w\equiv0$ in (\ref{am1})).

\begin{theorem}\label{1d_lb:thm}
 If a control algorithm $\A$ has finite $\ell_2$-gain bounds specified by $\gamma: [-M, M] \to [0, \infty)$ with $h=0$, for all $a \in [-M, M]$ and $f_t,w_t,x_t\in\R$ satisfying \eqref{am1}, then 
$ \gamma(a) \ge \max\{|a-M|,|a+M|\}/8\ge M/8$ for all $a\in [-M, M]$, and therefore $\ltgain(\A)\ge M/8$.
\end{theorem}

The result of Thm.~\ref{1d_lb:thm} suggests that the closed loop
$\ltgain$, no matter which adaptive controller is used, if it obtains finite $\ltgain$ for all systems satisfying the parametric uncertainty\xc{check}, must grow 
linearly with the parametric uncertainty size for all values of 
the uncertain parameter.
In particular, this makes it impossible to sacrifice performance at 
some values of $a$ to gain much improvement at other values of $a$.

\subsection{Thm.~\ref{1d_lb:thm} Proof Sketch}
In the analysis of Thm.~\ref{1d_lb:thm} we view the interaction between the control $u_t$  and disturbance $f_t$ as a game, where both are functions of past states and actions, but $u_t$ is chosen to minimize the $\ell_2$-gain bound, while $f_t$ is chosen to maximize it.

The proof considers the normalized version of the game where the state is instead $(\beta_t, z_t, \theta_t)$, with the following definitions:
\[ \beta_t=\frac{\sum_{s=0}^{t-1}x_s(x_{s+1}-u_s)}{\sum_{s=0}^{t-1}x_s^2},\qquad z_t=\frac{x_t}{\sqrt{\sum_{s=0}^{t-1}x_s^2}},\] 

$$\theta_t=\frac{(\sum_{s=0}^{t-1}(x_{s+1}-u_s)^2)(\sum_{s=0}^{t-1}x_s^2)-(\sum_{s=0}^{t-1}x_s(x_{s+1}-u_s))^2}{(\sum_{s=0}^{t-1}x_s^2)^2}.$$
Additionally, define the signals as follows,
$
\delta_t=\frac{u_t+\beta_tx_t}{\sqrt{\sum_{s=0}^{t}x_s^2}},\ 
 \nu_t=\frac{x_{t+1}-u_t-\beta_tx_t}{\sqrt{\sum_{s=0}^{t}x_s^2}}.
$
Then the states satisfy the following dynamics
\begin{align*}
z_{t+1}=\nu_t+\delta_t,\qquad
\beta_{t+1}=\beta_t+\frac{z_t\nu_t}{\sqrt{1+z_t^2}},\qquad
\theta_{t+1}=\frac{\theta_t+\nu_t^2}{1+z_t^2}.
\end{align*}
The game between $u$ and $f$ can now be interpreted as the game between
$\delta$ and $\nu$ where the normalized controller seeks to satisfy
$\gamma(a)^2 [(a - \beta_t)^2 + \theta_t] \ge 1$. Up to smaller order terms, we show that for any $a\in [-M, M]$, no matter what normalized control $\delta_t$ is used, there exists
\begin{itemize}
\item[(A)] An adversary strategy $\nu_t$ such that $\theta_t\to0$,
while $\beta_t$ stays (for sufficiently large $t$) 
within the interval $I_0 = [a+4\gamma(a),a+8\gamma(a)]$. 
\item[(B)]  An adversary strategy $\nu_t$ such that $\theta_t\to0$,
while $\beta_t$ stays (for sufficiently large $t$) 
within the interval $I_0= [a-8\gamma(a),a-4\gamma(a)]$.
\end{itemize}
Combining (A) and (B) 
assures that for
all $a\in[-M,M]$, the value of $8\gamma(a)$ cannot be 
smaller than the distance from $a$ to
either end of $[-M,M]$. Otherwise for iteration $\tau$ where $\beta_\tau\in [a-8\gamma(a),a-4\gamma(a)]$ or $\beta_\tau\in [a+4\gamma(a),a+8\gamma(a)]$, no finite $\gamma(\beta_\tau)$ can satisfy the constraint with $a=\beta_\tau$, and thus we have a 
desired lower bound for $\gamma(a)$. For a complete analysis, see App.~\ref{1d_lb_proof:sec}.

%  \xc{shorten this proof sketch} In the analysis of Thm.~\ref{1d_lb:thm} we view the interaction between the control $u_t$  and disturbance $f_t$ as a game, where controls are decided based on all state observations $x_s$ in order to maintain
% \vspace{-3mm}
% \begin{align*}
%     \gamma^2 [p_t a^2 - 2 q_ta + r_t] = \gamma^2 \sum_{s=0}^{t-1} f_t^2 \ge p_t~, 
% \end{align*}
% \vspace{-5mm}
% where, we define
% \[ \xi_t=x_{t+1}-u_t,\qquad p_t=\sum_{s=0}^{t-1}x_s^2,\qquad 
% q_t=\sum_{s=0}^{t-1}x_s(x_{s+1}-u_s),\qquad r_t=\sum_{s=0}^{t-1}\xi_s^2.\]

% In the above expression, $\gamma$ is an upper bound on the $\ltgain$ by definition.  The first step is to translate the
% game into a normalized version.  In particular, we work with the {\sl normalized} versions 
% $\delta_t$, $\nu_t$, $z_t$ of $u_t$, $\xi_t$, $x_t$, as well as additional signals
% $\beta_t$, $\theta_t$. Let $t_0$ be the smallest $t\in\mathbb Z_+$ such that $p_t>0$.
% For $t\ge t_0$ let
% \[ \beta_t=\frac{q_t}{p_t},\qquad\theta_t=\frac{r_tp_t-q_t^2}{p_t^2},\qquad
% z_t=\frac{x_t}{\sqrt{p_t}},\qquad\delta_t=\frac{u_t+\beta_tx_t}{\sqrt{p_t+x_t^2}},\qquad
% \nu_t=\frac{\xi_t-\beta_tx_t}{\sqrt{p_t+x_t^2}}.\]
% Since $x_t,\xi_t,u_t,p_t,q_t,r_t$ satisfy equations
% \[  x_{t+1}=\xi_t+u_t,~p_{t+1}=p_t+x_t^2,~q_{t+1}=q_t+x_t\xi_t,~r_{t+1}=r_t+\xi_t^2,\]
% $\delta_t$, $\nu_t$, $z_t$, $\beta_t$, $\theta_t$, for $t\ge t_0$, satisfy
% \begin{align*}
% z_{t+1}=\nu_t+\delta_t,\qquad
% \beta_{t+1}=\beta_t+\frac{z_t\nu_t}{\sqrt{1+z_t^2}},\qquad
% \theta_{t+1}=\frac{\theta_t+\nu_t^2}{1+z_t^2}.
% \end{align*}
% The game between $u$ and $f$ can now be interpreted as the game between
% $\delta$ and $\nu$ where the normalized controller seeks to satisfy
% $\gamma^2 [(a - \beta_t)^2 + \theta_t] \ge 1$. Up to smaller order terms, we show that,
% \begin{itemize}
% \item[(A)] An appropriate adversary strategy $\nu_t$, 
% assures that $\theta_t\to0$,
% while $\beta_t$ stays (for sufficiently large $t$) 
% within the interval $I_0 = [a+4\gamma,a+8\gamma]$,
% no matter which normalized control algorithm $\delta_t$ is used. 
% \item[(B)]  An appropriate adversary strategy $\nu_t$, 
% assures that $\theta_t\to0$,
% while $\beta_t$ stays (for sufficiently large $t$) 
% within the interval $I_0= [a-8\gamma,a-4\gamma]$,
% no matter which normalized control algorithm $\delta_t$ is used.
% \end{itemize}
% Combining assertions (A) and (B) 
% assures that for
% all $a\in[-M,M]$, the value of $8\gamma$ cannot be 
% smaller than the distance from $a$ to
% either end of the $[-M,M]$ interval endpoints, implying the 
% desired lower bound for $\gamma$.

% To achieve this, the adversary pursues the following three objectives:
% \begin{itemize}
% \item[(a)] keep $|z_t|\ge2\gamma$ at all times;
% \item[(b)] force $\beta_t\in I_0$, eventually;
% \item[(c)] make $\nu_t=0$ when objectives (a) and (b) are satisfied.
% \end{itemize}


\subsection{Upper Bound}
In this section, we show that, for $h<1/2$, 
the so-called {\sl certainty equivalence controller}
achieves an upper bound for the closed loop $\ell_2$ gain
which grows linearly with $M$. This
is remarkable, as a large $\ltgain$ is usually associated with low robustness
to uncertain dynamical feedback, with an expectation that a system with $\ltgain$ 
$\gamma$ can be destabilized by a feedback with 
$\ltgain$ of $1/\gamma$ (which is
certainly true for {\sl linear time invariant} systems). Since, with $h=0$, $\ltgain$
of the closed loop is shown to be at least $M/8$, one would expect that 
some uncertainty
$\mathbf\Delta$ of $\ltgain$ $h=8M^{-1}$ would destabilize the
system, but this is evidently not happening: 
according to Thm.~\ref{cert_equiv:thm} below, all uncertainty $\ltgain$s below $h=0.5$ are
well tolerated by the certainty equivalence controller (Alg.~\ref{alg:cert_equiv}).


\begin{algorithm2e}[h]

\label{alg:cert_equiv}
\KwIn{Time horizon $T$, system upper bound parameter $M$.}
Initialize $x_0 , u_0 =0$\\
\For{$t=1\dots T$}{
Observe $x_t$ and define $\tilde{z}_{t-1}(\hat{a}) = x_t -\hat{a} x_{t-1} - u_{t-1}$.\\
Compute $\bar{a}_t = \argmin_{\hat{a}} \sum_{s=0}^{t-1} \tilde{z}^2_s(\hat{a})$\\
Compute $\hat{a}_t = \text{clip}_{[-M, M]}(\bar{a}_t)$\\
Execute $u_t = -\hat{a}_t x_t$.
}
\caption{Certainty Equivalence Control}
\end{algorithm2e}


\vskip4mm\noindent

\begin{theorem}
\label{cert_equiv:thm}
 For $M\ge1/4$, with a system satisfying condition \eqref{am1} with $h<1/2$, Alg.~\ref{alg:cert_equiv} has
 \begin{align*}
     \ltgain(\A) \le \frac{(64M^2-8h)^{1/2}}{(1-2h)^{3/2}}~.
 \end{align*}
\end{theorem}

We provide an intuitive explanation why certainty equivalence can provide an $\ltgain$ bound.  If the algorithm estimates $\hat{a}$ inaccurately, strong convexity of the one dimensional least squares objective implies that the magnitude of the disturbances is a nontrivial fraction of the magnitude of the states up to that point.  On the other hand, if $\hat{a}_{t+1}$ is an accurate estimate of $a$, we can bound $\|x_{1:t}\|^2_2$ using the stability of the closed loop dynamics.  An $\ltgain$ bound follows from stitching these regimes together.  While we would like to extend these ideas to high dimensions, we note that the least squares objective is no longer strongly convex in such a setting.  In particular, $\|A-\hat{A}_t\|_2$ can be large in a direction where disturbances are small relative to the magnitude of the state.   A more technical approach that yields the tighter bound  of Thm.~\ref{cert_equiv:thm} can be found in App.~\ref{cert_equiv_proof:sec}.

\ug{TODO: " I find this explanation to be a bit too informal, and think that it could have been improved by a minimal use of formulas. E.g., I am not exactly sure what you mean by "nontrivial fraction", and how the estimate of "a" can help in controlling the closed-loop dynamics---I guess "good estimate" is defined relative to the magnitude of h, but this is not very clear here. Also, I miss an intuition regarding the precise role of h = 1/2.
"-ALT}

